A New Approach to Determine the Minimal Polynomials of Binary Modified de Bruijn Sequences

A binary modified de Bruijn sequence is an infinite and periodic binary sequence derived by removing a zero from the longest run of zeros in a binary de Bruijn sequence. The minimal polynomial of the modified sequence is its unique least-degree characteristic polynomial. Leveraging on a recent characterization, we devise a novel general approach to determine the minimal polynomial. We translate the characterization into a problem of identifying a Hamiltonian cycle in a specially constructed graph. Along the way, we demonstrate the usefullness of computational tools from the cycle joining method in the modified setup.

==> minpoly <==
% Encoding: UTF-8

@Article{Huber90,
  author  = {K. Huber},
  title   = {Some comments on Zech's logarithms},
  journal = {IEEE Trans. Inform. Theory},
  year    = {1990},
  volume  = {36},
  number  = {4},
  month   = {Jul},
  pages   = {946-950},
}

@ARTICLE{MS15,
author={J. Mykkeltveit and J. Szmidt},
journal={Contemporary Mathematics},
title={On cross joining de {B}ruijn sequences},
year={2015},
volume={632},
pages={333--344},
}

@Article{HK91,
  author  = {T. Helleseth and T. Klove},
  title   = {The number of cross-join pairs in maximum length linear sequences},
  journal = {IEEE Trans. Inform. Theory},
  year    = {1991},
  volume  = {37},
  number  = {6},
  month   = {Nov},
  pages   = {1731-1733},
}

@InBook{Taleb10,
  author    = {Taleb, Anas Abu and Mathew, Jimson and Pradhan, Dhiraj K.},
  title     = {Clustered De {B}ruijn Based Multi Layered Architectures for Sensor Networks},
  booktitle = {Recent Trends in Wireless and Mobile Networks: Second International Conference, WiMo 2010, Ankara, Turkey, June 26-28, 2010. Proceedings},
  year      = {2010},
  editor    = {{\"O}zcan, Abdulkadir and Chaki, Nabendu and Nagamalai, Dhinaharan},
  publisher = {Springer Berlin Heidelberg},
  pages     = {123--136},
  address   = {Berlin, Heidelberg},
}

@Article{Li2017,
author="Li, Ming
and Jiang, Yupeng
and Lin, Dongdai",
title="The adjacency graphs of some feedback shift registers",
journal="Designs, Codes and Cryptography",
year="2017",
volume="82",
number="3",
pages="695--713"
}


@article{mingli16,
author={Ming Li and Dongdai Lin},
title={Adjacency graphs, irreducible polynomials and cyclotomy},
year={2016},
url={http://eprint.iacr.org/2016/393},
}

@book{Menezes:1996,
 author = {Menezes, Alfred J. and Vanstone, Scott A. and Oorschot, Paul C. Van},
 title = {Handbook of Applied Cryptography},
 year = {1996},
 edition = {1st},
 publisher = {CRC Press, Inc.},
 address = {Boca Raton, FL, USA},
} 

@article{Chan82,
title = "On the complexities of de {B}ruijn sequences",
journal = "J. Combinat. Theory, Ser. A",
volume = "33",
number = "3",
pages = "233--246",
year = "1982",
author = "Agnes Hui Chan and Richard A Games and Edwin L Key",
}

@book{GG05,
author={Golomb, Solomon W. and Gong, Guang},
title={Signal Design for Good Correlation: for Wireless Communication, Cryptography, and Radar},
year={2004},
publisher={Cambridge Univ. Press},
address={New York},
}

@book{LN97,
title="Finite Fields",
author="Lidl, Rudolf and Niederreiter, Harald",
series="Encyclopaedia of Mathematics and Its Applications",
publisher="Cambridge Univ. Press",
address="New York",
year=1997
}

@article{Hemmati84,
 author = {Hemmati, Farhad and Schilling, Donald L. and Eichmann, George},
 title = {Adjacencies Between the Cycles of a Shift Register with Characteristic Polynomial $(1+x)^{n}$},
 journal = {IEEE Trans. Comput.},
 year = {1984},
 volume = {33},
 number = {7},
 month = {Jul},
 issn = {0018-9340},
 pages = {675--677},
 publisher = {IEEE Computer Society},
}

@Article{M72,
  author  = {Johannes Mykkeltveit},
  title   = {A proof of {G}olomb's conjecture for the de {B}ruijn graph},
  number  = {1},
  pages   = {40 - 45},
  volume  = {13},
  journal = {J. of Combinat. Theory, Ser. B},
  year    = {1972},
}

@book{Nath00,
  title={Elementary Methods in Number Theory},
  author={Nathanson, M.B.},
  isbn={9780387989129},
  series={Graduate Texts in Mathematics},
  year={2000},
  publisher={Springer},
  address={New York}
}

@book{Storer67,
title={Cyclotomy and Difference Sets},
author={Storer, T.},
series={Lectures in Advanced Mathematics},
year={1967},
publisher={Markham Pub. Co.},
address={Chicago, USA}
}
{{B}ruijn46,
  author  = {de {B}ruijn, N. G.},
  title   = {A Combinatorial Problem},
  journal = {Koninklijke Nederlandse Akademie v. Wetenschappen},
  year    = {1946},
  volume  = {49},
  pages   = {758--764},
}

@Article{EtzionLempel84,
  author  = {T. Etzion and A. Lempel},
  title   = {Algorithms for the generation of full-length shift-register sequences},
  number  = {3},
  pages   = {480--484},
  volume  = {30},
  journal = {IEEE Trans. Inform. Theory},
  month   = {May},
  year    = {1984},
}

@Article{Fred82,
  author  = {Harold Fredricksen},
  title   = {A Survey of Full Length Nonlinear Shift Register Cycle Algorithms},
  number  = {2},
  pages   = {195--221},
  volume  = {24},
  journal = {SIAM Rev.},
  year    = {1982},
}

@article{HH96,
author={Erik R. Hauge and Tor Helleseth},
title={De {B}ruijn sequences, irreducible codes and cyclotomy},
journal={Discrete Math.},
volume={159},
number={1-3},
pages={143-154},
year={1996},
}

@Article{HM96,
  author  = {Erik R. Hauge and Johannes Mykkeltveit},
  title   = {On the classification of de {B}ruijn sequences},
  number  = {1–3},
  pages   = {65 - 83},
  volume  = {148},
  journal = {Discrete Math.},
  year    = {1996},
}

@book{Knuth4A,
   title = "The Art of Computer Programming. Vol.~4A., Combinatorial Algorithms. Part 1",
   author = "Knuth, Donald Ervin",
   publisher = "Addison-Wesley",
   address = "Upple Saddle River (N.J.), London, Paris",
   note = "",
   year = 2011
}

@ARTICLE{KSSK00, 
author={K. Kurosawa and F. Sato and T. Sakata and W. Kishimoto}, 
journal={IEEE Trans. Inform. Theory}, 
title={A relationship between linear complexity and k-error linear complexity}, 
year={2000}, 
volume={46}, 
number={2}, 
pages={694-698}, 
month={Mar}
}

@ARTICLE{Lempel70, 
author={A. Lempel}, 
journal={IEEE Trans. on Computers}, 
title={On a Homomorphism of the de {B}ruijn Graph and its applications to the design of feedback shift registers}, 
year={1970}, 
volume={C-19}, 
number={12}, 
pages={1204--1209}, 
month={Dec}
}

@ARTICLE{Li14-1, 
author={C. Li and X. Zeng and T. Helleseth and C. Li and L. Hu}, 
journal={IEEE Trans. Inform. Theory}, 
title={The Properties of a Class of Linear {FSR}s and Their Applications to the Construction of Nonlinear {FSR}s}, 
year={2014}, 
volume={60}, 
number={5}, 
pages={3052-3061}, 
month={May}
}

@ARTICLE{Li14-2, 
author={C. Li and X. Zeng and C. Li and T. Helleseth}, 
journal={IEEE Trans. Inform. Theory}, 
title={A Class of de {B}ruijn Sequences}, 
year={2014}, 
volume={60}, 
number={12}, 
pages={7955-7969}, 
month={Dec}
}

@ARTICLE{Li16, 
author={C. Li and X. Zeng and C. Li and T. Helleseth and M. Li}, 
journal={IEEE Trans. Inform. Theory}, 
title={Construction of de {B}ruijn Sequences From {LFSR}s With Reducible Characteristic Polynomials}, 
year={2016}, 
volume={62}, 
number={1}, 
pages={610-624},
month={Jan}
}

@Inbook{OB15,
author="Orenstein, Yaron
and Berger, Bonnie",
editor="Pop, Mihai
and Touzet, H{\'e}l{\`e}ne",
chapter="Efficient Design of Compact Unstructured RNA Libraries Covering All k-mers",
title="Algorithms in Bioinformatics: 15th International Workshop, WABI 2015, Atlanta, GA, USA, September 10-12, 2015, Proceedings",
year="2015",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="308--325",
}

@article{NP13,
author = {Nagarajan, Niranjan and Pop, Mihai},
journal = {Nature Reviews Genetics},
keywords = {bioinformatics genome sequencing},
number = 3,
pages = {157--167},
publisher = {Nature Publishing Group},
title = {Sequence assembly demystified},
volume = 14,
year = 2013
}

@article{PTW01,
  author = {Pevzner, Pavel A. and Tang, Haixu and Waterman, Michael S.},
  journal = {Proceedings of the National Academy of Sciences},
  keywords = {euler sequencing short-reads},
  number = 17,
  pages = {9748-9753},
  title = {An {E}ulerian path approach to {DNA} fragment assembly},
  volume = 98,
  year = 2001
}

@Article{Ral82,
  author    = {Anthony Ralston},
  title     = {De {B}ruijn Sequences - A Model Example of the Interaction of Discrete Mathematics and Computer Science},
  journal   = {Math. Mag.},
  year      = {1982},
  volume    = {55},
  number    = {3},
  pages     = {131-143},
  publisher = {Mathematical Association of America},
}

@ARTICLE{SG13, 
author={S. Spinsante and E. Gambi}, 
journal={IEEE Aerospace and Electronic Systems Magazine}, 
title={De {B}ruijn binary sequences and spread spectrum applications: A marriage possible?}, 
year={2013}, 
volume={28}, 
number={11}, 
pages={28-39}, 
ISSN={0885-8985}, 
month={Nov},}

@InProceedings{KRR14,
    author={Kociumaka, Tomasz and Radoszewski, Jakub and Rytter, Wojciech},
    title = {Computing k-th {L}yndon Word and Decoding Lexicographically Minimal de {B}ruijn Sequence},
    booktitle = {Combinatorial Pattern Matching: Proceedings of 25th Annual Symposium, CPM 2014},
    month = Jun,
    year = 2014,
    publisher = {Springer International},
    editor = {Kulikov, Alexander S.
and Kuznetsov, Sergei O.
and Pevzner, Pavel},
    pages = {202--211},
}

@article{KKS15,
  author    = {Swastik Kopparty and
               Mrinal Kumar and
               Michael E. Saks},
  title     = {Efficient indexing of necklaces and irreducible polynomials over finite
               fields},
  journal   = {Electronic Colloquium on Computational Complexity {(ECCC)}},
  volume    = {22},
  pages     = {47},
  year      = {2015},
}

@InProceedings{MG13,
  author    = {Mandal, Kalikinkar and Gong, Guang},
  title     = {Cryptographically Strong de {B}ruijn Sequences with Large Periods},
  booktitle = {Selected Areas in Cryptography},
  year      = {2013},
  editor    = {Knudsen, Lars R. and Wu, Huapeng},
  publisher = {Springer Berlin Heidelberg},
  isbn      = {978-3-642-35999-6},
  pages     = {104--118},
  address   = {Berlin, Heidelberg},
}

@Article{Mayhew00,
  author   = {G.L Mayhew},
  title    = {Clues to the hidden nature of de {B}ruijn sequences},
  journal  = {Comput. Math. Appl.},
  year     = {2000},
  volume   = {39},
  number   = {11},
  pages    = {57 - 65},
}

@Article{Jacobi,
  author   = {Jacobi, C.G.J.},
  title    = {\"{U}ber die Kreistheilung und ihre Anwendung auf die Zahlentheorie.},
  journal  = {Journal f\"{u}r die reine und angewandte Mathematik},
  year     = {1846},
  language = {ger},
  volume   = {30},
  pages    = {166-182},
}

@Article{Alh12,
  author  = {Abbas Alhakim},
  title   = {Spans of preference functions for de {B}ruijn sequences},
  journal = {Discrete Appl. Math.},
  year    = {2012},
  volume  = {160},
  number  = {7},
  pages   = {992 - 998},
}

@Unpublished{WWZ18,
  author = {Wang, Xiaofang and Wong, Dennis and Zhang, Wei Guo},
  title  = {A simple greedy de {B}ruijn sequence construction},
  year   = {2018},
}

@Article{SWW16,
  author  = {Joe Sawada and Aaron Williams and Dennis Wong},
  title   = {Generalizing the Classic Greedy and Necklace Constructions of de {B}ruijn Sequences and Universal Cycles},
  journal = {Electr. J. Comb.},
  year    = {2016},
  volume  = {23},
  number  = {1},
  pages   = {P1.24},
}

@Article{Sawada17,
  author  = {Joe Sawada and Aaron Williams and Dennis Wong},
  title   = {A simple shift rule for $k$-ary de {B}ruijn sequences},
  journal = {Discrete Math.},
  year    = {2017},
  volume  = {340},
  number  = {3},
  pages   = {524--531},
}

@Article{Dragon18,
  author  = {Patrick Baxter Dragon and Oscar I. Hernandez and Joe Sawada and Aaron Williams and Dennis Wong},
  title   = {Constructing de {B}ruijn sequences with co-lexicographic order: The $k$-ary Grandmama sequence},
  journal = {Eur. J. Comb.},
  year    = {2018},
  volume  = {72},
  pages   = {1--11},
}

@Article{RuskeySW12,
  author    = {Frank Ruskey and Joe Sawada and Aaron Williams},
  title     = {De {B}ruijn Sequences for Fixed-Weight Binary Strings},
  journal   = {{SIAM} J. Discrete Math.},
  year      = {2012},
  volume    = {26},
  number    = {2},
  pages     = {605--617},
}

@Article{Martin34,
  author  = {M. H. Martin},
  title   = {A problem in arrangements},
  journal = {Bull. Am. Math. Soc},
  year    = {1934},
  volume  = {40},
  number  = {12},
  month   = {Dec},
  pages   = {859--865},
}

@Article{Bruijn46,
  author  = {de Bruijn, N. G.},
  title   = {A Combinatorial Problem},
  journal = {Koninklijke Nederlandse Akademie v. Wetenschappen},
  year    = {1946},
  volume  = {49},
  pages   = {758--764},
}

@Article{Gabric18,
  author    = {Daniel Gabric and Joe Sawada and Aaron Williams and Dennis Wong},
  title     = {A framework for constructing de Bruijn sequences via simple successor rules},
  journal   = {Discrete Math.},
  year      = {2018},
  volume    = {341},
  number    = {11},
  month     = {Nov},
  pages     = {2977--2987},
  publisher = {Elsevier {BV}},
}

@Book{Golomb,
  author    = {Golomb, Solomon W},
  title     = {Shift Register Sequences},
  year      = {2017},
  edition   = {3rd Revised},
  publisher = {World Scientific},
  city      = {#Singapore#},
}

@Article{GS18,
  author   = {Daniel Gabric and Joe Sawada},
  title    = {Constructing de Bruijn sequences by concatenating smaller universal cycles},
  journal  = {Theoretical Computer Science},
  year     = {2018},
  volume   = {743},
  pages    = {12 - 22},
}

@Article{Sawada16,
  author    = {Joe Sawada and Aaron Williams and Dennis Wong},
  title     = {A surprisingly simple de {B}ruijn sequence construction},
  journal   = {Discrete Math.},
  year      = {2016},
  volume    = {339},
  number    = {1},
  month     = {jan},
  pages     = {127--131},
  publisher = {Elsevier {BV}},
}

@Article{Huang90,
  author  = {Yuejiang Huang},
  title   = {A new algorithm for the generation of binary de Bruijn sequences},
  journal = {J. Algorithms},
  year    = {1990},
  volume  = {11},
  number  = {1},
  pages   = {44 - 51},
}

@Book{Tutte,
  author    = {Tutte, W.T.},
  title     = {Graph Theory},
  year      = {2001},
  series    = {Cambridge Mathematical Library},
  publisher = {Cambridge University Press},
}

@InProceedings{PM06,
  author    = {George Petrides and Johannes Mykkeltveit},
  title     = {On the Classification of Periodic Binary Sequences into Nonlinear Complexity Classes},
  booktitle = {Sequences and Their Applications - {SETA} 2006, 4th Int. Conf., Beijing, China, September 24-28, 2006, Proceedings},
  year      = {2006},
  pages     = {209--222},
}

@PhdThesis{Jansen89,
  author = {Jansen, Cees J.~A.~},
  title  = {Investigations on nonlinear stream cipher systems: Construction and evaluation methods},
  year   = {1989},
  school = {Technical University of Delft},
}

@Article{Chang2019,
  author  = {Chang, Zuling and Ezerman, Martianus Frederic and Ling, San and Wang, Huaxiong},
  title   = {On binary de {B}ruijn sequences from {LFSRs} with arbitrary characteristic polynomials},
  number  = {5},
  pages   = {1137--1160},
  volume  = {87},
  journal = {Des. Codes, Cryptogr.},
  month   = {May},
  year    = {2019},
}

@Article{Fred72,
  author    = {Harold Fredricksen},
  title     = {Generation of the {F}ord sequence of length $2n$, $n$ large},
  number    = {1},
  pages     = {153--154},
  volume    = {12},
  journal   = {J. Combinat. Theory, Ser. A},
  month     = {Jan},
  publisher = {Elsevier {BV}},
  year      = {1972},
}

@Article{Gabric20,
  author  = {D. Gabric and J. Sawada and A. Williams and D. Wong},
  title   = {A successor rule framework for constructing $k$-ary de {Bruijn} sequences and universal cycles},
  number  = {1},
  pages   = {679--687},
  volume  = {66},
  journal = {IEEE Trans. Inform. Theory},
  month   = {Jan},
  year    = {2020},
}

@InCollection{Buss2019,
  author    = {Sam Buss and Alexander Knop},
  title     = {Strategies for Stable Merge Sorting},
  booktitle = {Proceedings of the Thirtieth Annual {ACM}-{SIAM} Symposium on Discrete Algorithms},
  year      = {2019},
  publisher = {Society for Industrial and Applied Mathematics},
  pages     = {1272--1290},
  month     = {Jan},
}

@InProceedings{McIlroy93,
  author    = {McIlroy, Peter},
  title     = {Optimistic Sorting and Information Theoretic Complexity},
  booktitle = {Proceedings of the Fourth Annual ACM-SIAM Symposium on Discrete Algorithms},
  year      = {1993},
  series    = {SODA '93},
  publisher = {Society for Industrial and Applied Mathematics},
  location  = {Austin, Texas, USA},
  pages     = {467--474},
  address   = {Philadelphia, PA, USA},
  numpages  = {8},
}

@Article{Jansen91,
  author    = {C.J.A. Jansen and W.G. Franx and D.E. Boekee},
  title     = {An efficient algorithm for the generation of {DeBruijn} cycles},
  journal   = {{IEEE} Trans. Inform. Theory},
  year      = {1991},
  volume    = {37},
  number    = {5},
  month     = {May},
  pages     = {1475--1478},
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
}

@Article{Booth80,
  author    = {Kellogg S. Booth},
  title     = {Lexicographically least circular substrings},
  journal   = {Inf. Process. Lett.},
  year      = {1980},
  volume    = {10},
  number    = {4-5},
  month     = {Jul},
  pages     = {240--242},
  publisher = {Elsevier {BV}},
}

@Electronic{timsort,
  author = {Peters, Tim},
  title  = {[Python-Dev] Sorting},
  url    = {https://mail.python.org/pipermail/python-dev/2002-July/026837.html},
}

@Article{Farhi,
  author  = {Bakir Farhi},
  title   = {An Identity Involving the Least Common Multiple of Binomial Coefficients and Its Application},
  journal = {Amer. Math. Monthly},
  year    = {2009},
  volume  = {116},
  number  = {9},
  pages   = {836--839},
}

@Book{Ding96,
  author    = {Ding, C. and Pei, D. and Salomaa, A.},
  title     = {Chinese Remainder Theorem: Applications in Computing, Coding, Cryptography},
  year      = {1996},
  publisher = {World Scientific Publishing Co., Inc.},
  address   = {USA},
}

@Book{Halmos,
  author    = {Halmos, P.R.},
  title     = {Naive Set Theory},
  publisher = {Springer New York},
  series    = {Undergraduate Texts in Mathematics},
  year      = {1974},
}

@Article{Chang2017,
  author       = {Zuling Chang and Martianus Frederic Ezerman and San Ling and Huaxiong Wang},
  year         = {2017-03},
  journal = {Cryptography and Communications},
  title        = {Construction of de Bruijn sequences from product of two irreducible polynomials},
  number       = {2},
  pages        = {251--275},
  volume       = {10},
  publisher    = {Springer Science and Business Media {LLC}},
}

@Article{Chang2020,
  author    = {Zuling Chang and Martianus Frederic Ezerman and Adamas Aqsa Fahreza},
  title     = {On greedy algorithms for binary de {Bruijn} sequences},
  url       = {https://doi.org/10.1007/s00200-020-00459-3},
  journal   = {Appl. Algebra Eng. Commun.},
  publisher = {Springer Science and Business Media {LLC}},
  year      = {2020},
}

@Article{Compeau2011,
  author       = {Phillip E C Compeau and Pavel A Pevzner and Glenn Tesler},
  year         = {2011-11},
  journal = {Nature Biotechnology},
  title        = {How to apply de Bruijn graphs to genome assembly},
  number       = {11},
  pages        = {987--991},
  volume       = {29},
  publisher    = {Springer Science and Business Media {LLC}},
}

@Article{Dong2019,
  author       = {Yu-Jie Dong and Tian Tian and Wen-Feng Qi and Zhong-Xiao Wang},
  year         = {2019-11},
  journal = {Finite Fields and Their Applications},
  title        = {New results on the minimal polynomials of modified de Bruijn sequences},
  pages        = {101583},
  volume       = {60},
  publisher    = {Elsevier {BV}},
}

@Article{Etzion1984,
  author       = {T. Etzion and A. Lempel},
  year         = {1984},
  journal      = {{IEEE} Trans. Inform. Theory},
  title        = {Construction of de {B}ruijn sequences of minimal complexity},
  number       = {5},
  month        = {Sep},
  pages        = {705--709},
  volume       = {30},
  publisher    = {Institute of Electrical and Electronics Engineers ({IEEE})},
}

@InProceedings{Gong2007,
  author    = {Gong, Guang},
  booktitle = {Sequences, Subsequences, and Consequences},
  year      = {2007},
  title     = {Randomness and Representation of Span n Sequences},
  editor    = {Golomb, Solomon W. and Gong, Guang and Helleseth, Tor and Song, Hong-Yeop},
  location  = {Berlin, Heidelberg},
  pages     = {192--203},
  publisher = {Springer Berlin Heidelberg},
}

@Article{Kyureghyan2008,
  author       = {Gohar M. Kyureghyan},
  year         = {2008},
  journal = {Discrete Appl. Math.},
  title        = {Minimal polynomials of the modified de {B}ruijn sequences},
  number       = {9},
  pages        = {1549--1553},
  volume       = {156},
  publisher    = {Elsevier {BV}},
}

@Article{StMarie1894,
  author  = {Camille Flye Sainte-Marie},
  title   = {Solution to question nr. 48},
  pages   = {107--110},
  volume  = {1},
  journal = {L'interm\'ediaire des Math\'ematiciens},
  year    = {1894},
}

@Article{Mayhew1990,
  author    = {G.L. Mayhew and S.W. Golomb},
  year      = {1990},
  title     = {Linear spans of modified de {B}ruijn sequences},
  number    = {5},
  month     = {Sep},
  pages     = {1166--1167},
  volume    = {36},
  journal   = {{IEEE} Trans. Inform. Theory},
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
}

@Book{Pless1998,
  author    = {Vera Pless},
  year      = {1998-06},
  title     = {Introduction to the Theory of Error-Correcting Codes},
  publisher = {John Wiley {\&} Sons, Inc.},
}

@Article{Tan2018,
  author  = {Lin Tan and Hong Xu and Wen-Feng Qi},
  title   = {Preliminary results on the minimal polynomial of modified de {Bruijn} sequences},
  pages   = {356-365},
  volume  = {50},
  journal = {Finite Fields Appl.},
  year    = {2018},
}

@Article{Wang2020,
  author    = {Hong-Yu Wang and Qun-Xiong Zheng and Zhong-Xiao Wang and Wen-Feng Qi},
  title     = {The minimal polynomials of modified de {Bruijn} sequences revisited},
  pages     = {101735},
  volume    = {68},
  journal   = {Finite Fields Appl.},
  publisher = {Elsevier {BV}},
  year      = {2020},
}

@online{OEIS,
  author={N. J. A. Sloane and {The OEIS Foundation Inc.}},
  title={The {O}nline {E}ncyclopedia of {I}nteger {S}equences},
  year={2020},
  url={https://oeis.org/A0001037},
} 

@Article{Kuhn2012,
  author  = {Daniela K\"uhn and Deryk Osthus},
  title   = {A survey on {Hamilton} cycles in directed graphs},
  number  = {5},
  pages   = {750-766},
  volume  = {33},
  journal = {Eur. J. Comb.},
  year    = {2012},
}

@Book{BangJensen2009,
  author    = {J{\o}rgen Bang-Jensen and Gregory Z. Gutin},
  title     = {Digraphs: Theory, Algorithms and Applications},
  edition   = {2nd ed.},
  location  = {London},
  publisher = {Springer-Verlag},
  year      = {2009},
}

@Article{Etzion99,
  author  = {T. {Etzion}},
  title   = {Linear complexity of de {Bruijn} sequences-old and new results},
  number  = {2},
  month   = {Mar},
  pages   = {693--698},
  volume  = {45},
  journal = {IEEE Trans. Inform. Theory},
  year    = {1999},
}

@Article{Good1946,
  author       = {I. J. Good},
  journal      = {J. London Math. Soc.},
  title        = {Normal Recurring Decimals},
  number       = {3},
  pages        = {167--169},
  volume       = {s1-21},
  month        = {Jul},
  publisher    = {Wiley},
  year         = {1946},
}

@Comment{jabref-meta: databaseType:biblatex;}

